Stitch: Step-by-step LLM Guided Tutoring for Scratch

Block-based environments such as Scratch are increasingly popular in programming education. While block syntax reduces surface errors, semantic bugs remain common and challenging for novices to resolve. Existing debugging workflows typically show the correct program directly to learners, a strategy that may fix errors but undermines the development of problem-solving skills. We present Stitch, an interactive tutoring system that replaces "showing the answer" with step-by-step scaffolding. The system's Diff-Analyze module contrasts a student's project with a reference implementation, identifies the most critical differences, and uses a large language model to explain why these changes matter. Learners inspect highlighted blocks through a custom rendering engine, understand the explanations, and selectively apply partial fixes. This iterative process continues until the intended functionality is achieved. We evaluate Stitch in an empirical study, comparing it against a state-of-the-art automated feedback generation tool for Scratch. Our key insight is that simply presenting the correct program is pedagogically ineffective. In contrast, our interactive, step-by-step guided system promotes a more effective learning experience. More broadly, what constitutes effective feedback in block-based programming remains an open question. Our evaluation provides new evidence that step-by-step tutoring significantly enhances learning outcomes, outperforming both direct-answer approaches and current automated feedback generation tools.

==> secs/compare.tex <==
\section{Comparative Analysis: \app and ViScratch \daming{this seems better placed after the evaluation section}}

To better understand the positioning of \app, we compare it with the recently proposed ViScratch system. Although both use LLM to assist with Scratch programming, there are fundamental differences in their positioning and design. 

ViScratch focuses on automatic debugging, aiming to enable AI to automatically diagnose and fix defects in student projects without teacher intervention. A typical application scenario is when a student's work contains errors or does not meet expected behavior. The system automatically provides a fix by analyzing the code and gameplay videos. \app, does not aim to automatically fix code, but instead provides interactive prompts to help students complete their projects. In other words, ViScratch can be considered an intelligent "debugger," while \app is more like an intelligent "tutor." This determines the differences in their design choices: ViScratch prioritizes the correctness and efficiency of fixes, such as ensuring a first-time fix success rate and minimizing code changes; \app emphasizes the effectiveness of guidance and the learning process, specifically whether the prompts allow students to understand the problem and learn to solve it.

\para{Different feedback methods}: After detecting a program defect, ViScratch directly generates a code-level patch solution and applies it to the project. It provides specific modification instructions in the form of an AST editor, allowing the code to be fixed directly. Students primarily act as observers, observing the system's resulting changes. In contrast, \app's feedback is presented in the form of dialog prompts, never directly providing complete code modification solutions. Even if the system "knows" the correct answer (derived from the target project's diffs), it exposes the problem to the student step-by-step, leaving the student to personally make the correction. This difference reflects two educational philosophies: ViScratch is more about "providing direct answers," while \app "provides guidance." While the patches ViScratch outputs are often small and easy to understand, they are still ready-made answers. \app, on the other hand, requires students to apply the ideas provided in the prompts to generate answers. This interactive feedback is more consistent with guided learning in teaching and is believed to effectively promote the internalization of knowledge by beginners.

\para{Learner Support}: \app was designed to simulate the step-by-step guidance provided by a real teacher, focusing on maintaining student initiative and engagement. The system uses multiple rounds of dialogue to ensure students remain engaged in problem solving, with each prompt building on the student's previous work. This is crucial for cultivating students' debugging habits and patience in problem-solving. While automated tools like ViScratch significantly reduce the burden of debugging, they also reduce the opportunity for students to identify and correct errors independently. Especially in youth programming education, if tools automatically correct problems as soon as they encounter them, students may find it difficult to develop the ability to troubleshoot independently. In this regard, \app offers a middle ground: apply AI's intelligent analytical capabilities while still allowing students to direct the correction process, achieving a balance between developing skills and achieving task completion.

In summary, \app's unique value lies in its deep integration of AI technology and instructional guidance. In contrast, while ViScratch and other approaches excel in automation and accuracy, they lack support for guided learning, which is a quite disadvantageous for programming beginners.

We believe that in the real classroom, fully automated error correction tools certainly save time, but guiding students to solve problems independently is more aligned with educational objectives. \app's step-by-step prompting mechanism has the potential to enable AI to not just replace students' thinking, but rather facilitate better thinking. This student-centered AI tutoring model is a valuable complement and enhancement to existing automated debugging tools.


